Learning a Tree-Structured Ising Model in Order to Make Predictions

We study the problem of learning a tree Ising model from samples such that subsequent predictions made using the model are accurate. The prediction task considered in this paper is that of predicting the values of a subset of variables given values of some other subset of variables. Virtually all previous work on graphical model learning has focused on recovering the true underlying graph. We define a distance ("small set TV" or ssTV) between distributions $P$ and $Q$ by taking the maximum, over all subsets $\mathcal{S}$ of a given size, of the total variation between the marginals of $P$ and $Q$ on $\mathcal{S}$; this distance captures the accuracy of the prediction task of interest. We derive non-asymptotic bounds on the number of samples needed to get a distribution (from the same class) with small ssTV relative to the one generating the samples. One of the main messages of this paper is that far fewer samples are needed than for recovering the underlying tree, which means that accurate predictions are possible using the wrong tree.

==> App-examples.tex <==
\section{Preliminaries and examples}
In this section we work through several examples in order to gain intuition for the main results stated in Theorems \ref{t:decomposition} and \ref{t:ssTVk}. We begin with a definition pertaining to restriction of a tree to a subset of nodes, which will be used both in this section and later on in the proofs.
%\GB{Theorem references}

\subsection{Canonical subtrees}
\label{ss:subtrees}
\begin{defn}
Given the tree $\T=(\VV,\EE)$ and the subset of nodes $\SS\subseteq{\VV}\,,$ we  define the \emph{induced subtree} $\T_{|\SS}$ to be the (simplified) subtree of $\T$ restricted to the nodes in $\SS$. 
$\T_{|\SS}$ is constructed as following: 

Step 1: Throw away all edges and nodes not appearing in a path between two nodes in $\SS\,.$

Step 2: Replace each path consisting entirely of degree two nodes not in $\SS$ by a single edge. 
\end{defn}

Note that the joint distribution over the nodes in $\SS$ can be achieved using this tree. By Markov property, throwing away the nodes not appearing in the paths between nodes in $\SS$ does not change the marginal distribution on $\SS\,.$ Additionally, we can replace any path consisting of degree two nodes not in $\SS$ by a single edge. The weight of this edge should be  adjusted such that the pairwise distribution between its end points (or equivalently their correlation) is the same as before.

%Step 2: Remove all the nodes $v$ such that $v\notin\SS$ and $v$ has degree two. Replace each path consisting entirely of removed degree two nodes by a single edge.
% removing all the degree two nodes in 
%$\T_{|\SS}$  contains all the nodes in $\SS$ and all the junction nodes that appear in the path between at least two pairs of nodes in $\SS$ according to $\T\,.$ The connectivity in $\T_{|\SS}$ is induced by the connectivity in $\T$ and the edges strength are defined to that the correlation along any edge in $\T_{|\SS}$ matches the correlation between corresponding nodes in $\T\,.$
\begin{defn}
Given the tree $\T=(\VV,\EE)$ and the set of nodes $\SS\subseteq{\VV}\,,$ we  define the set of \emph{junction nodes} $\mathcal{J}_\SS$  to be the set of nodes $j\in\T_{|\SS}$ and $j\notin\SS$ which have degree 3 or higher.
%$\mathcal{J}_\SS=\{j\in\T_{|\SS}; j\notin\SS\,, \exists u,u'v,v'\in\SS \text{such that} j\in\path_{\T_{|\SS}}(u,u')\cap\path_{\T_{|\SS}}(v,v') \}\,.$
\end{defn}

The construction of $T_{|\SS}$ just outlined is similar to the one described in \cite{mossel2013robust,erdos1999few}.
\begin{defn} [Cherry] \label{def:cherry}
A cherry is a subtree consisting of a node (called the parent) and exactly two leaves (children). Note that the leaves must be adjacent to the parent.\end{defn}


\begin{defn}
Given the tree $\T\,,$ a \textit{canonical subtree} of nodes in $\SS$ is a subtree that 1) has $\SS$ in its leaves and 2) has junction nodes of degree 3.%, and 3)for all $u,v\in\SS\,,$ there exists $j\in\mathcal{J}_{\SS}$ such that $j\in\path_{\T_{\S}}(u,v)\,.$
\end{defn}
%Note that the canonical subtrees are determined up to automorphism using the  
Note that the canonical subtree over a given set of nodes is not necessarily unique. 
We use canonical subtrees to prove the main result in Theorem~\ref{t:decomposition}. In Section~\ref{s:proofDecomposition} it is shown by induction that any subtree over a set of nodes can be equivalently represented with a canonical subtree (possibly via introducing some virtual nodes). Some examples of this procedure will be given in Section~\ref{s:examples}.

We show that there is always a cherry (defined in Definition~\ref{def:cherry}) in the canonical subtree with the leaves $\{i,j\}$ in $\SS$ and the parent node $u\notin\SS\,.$ Due to the Markov property, the random variables associated with the leaves of the cherry $X_i,X_j$ are conditionally independent of $X_{\SS\setminus\{i,j\}}$ given $X_u\,.$ This underlies the induction argument for the proof of Equation~\eqref{e:decomposition}.

\subsection{Examples}\label{s:examples}

The following sections apply Theorem \ref{t:decomposition} to find the marginals of size two, three and four in a tree. 


\begin{ex}[Marginal on two nodes] \label{ex:k2}
Let $\SS=\{1,2\}$ without loss of generality. For any tree $\T\,,$ the subtree $\T_{|\SS}$ is simply an edge between the nodes $(1,2)$. This is also the unique canonical subtree over the set of nodes with cardinality 2. Since $P(x_1,x_2)  = \frac{1}{4}[1+x_1x_2 \mu_{12}]\,,$ the marginal over two nodes satisfies the form given in Equation~\eqref{e:decomposition}.
\end{ex}

\begin{ex}[Marginal on three nodes] \label{ex:k3}
Let $\SS=\{1,2,3\}$. For any tree $\T\,,$ the subtree $\T_{|\SS}$ is automorphic to either of the two trees $\T_1$ or $\T_2$ given in Figure~\ref{fig:marginalTrees}. 
The tree $\T_2$ is the unique canonical subtree over $\SS\,.$

Any marginal distribution represented according to $\T_1$ or its automorphism can also be represented by the tree $\T_2\,.$ As an example, if $X_1\to X_2\to X_3$ form a Markov chain according to $\T_1\,,$ then we can define a virtual node $u$ such that $\Ex_{P}X_2X_u=1\,$ and $X_1,X_2,X_3,X_u$ are represented by tree $\T_2\,.$
Using Lemma \ref{l:marginal3} whether $P(x_\SS)$ is distributed according to $\T_1$ or $\T_2\,,$ the following holds:
\begin{align} \label{eq:k3}
P(x_1,x_2,x_3) & = \frac{1}{2^3} \bigg( 1+ \sum_{\substack{\{i,j\}\subseteq\{1,2,3\}\\ i\neq j}} x_i x_j \mu_{ij}\bigg)
\end{align}
\end{ex}

\begin{figure}[t]
  \centering
\includegraphics[width=4in]{figK.pdf}
  \caption{$\T_1$ and $\T_2$ are all possible subtrees over nodes $\{1,2,3\}$ (up to automorphism). Any distribution over $\T_1$ can be represented using $\T_2$ as well. $\T_3, \T_4, \T_5$ and $\T_6$ are all possible subtrees over nodes $\{1,2,3,4\}$ (up to automorphism). All distributions over $\T_3, \T_4$ and $\T_5$ can be represented using $\T_6\,.$ We call $\T_{6}$ the quartet over $(12|34)$}
  \label{fig:marginalTrees}
\end{figure}

%\begin{ex}[k=3]\label{ex:k3}
%Given tree $\T$ and nodes $\SS=\{1,2,3\}\,,$ the subtree $\T_{|\SS}$ can take two different forms. Either the random variables $X_1, X_2$ and $X_3$ form a Markov chain (as in Figure )
%\end{ex}

\begin{ex}[Marginal on four nodes]\label{ex:k4}
For $\SS=\{1,2,3,4\}$, there exist four possible induced subtrees $\T_3,\T_4,\T_5$ and $\T_6$ up to automorphism shown in Figure~\ref{fig:marginalTrees}. 
Note that the canonical subtree is not unique. Both quartets $(12|34)$ (i.e., $\T_6$ in Figure~\ref{fig:marginalTrees}), $(13|24)$ and $(14|23)$ are canonical subtrees for $\SS=\{1,2,3,4\}\,.$

 Similar to the example given for $|\SS|=3\,,$ all distributions represented by $\T_3, \T_4$ and $\T_5$ and their automorphism can be represented by either the quartet structure $(12|34)\,,(13|24)$ or $(14|23)\,$ by possibly using virtual nodes $u$ and/or $v$. For example, when $P(x_{\SS})$ is represented by $\T_3$, one can define virtual nodes $u$ and $v$ to represent $P(x_\SS)$ on $\T_6$ such that $\mu_{2u} = \mu_{v3}=1$ and consequently $ \mu_{1u}=\mu_{2u}\,, \mu_{uv}=\mu_{23}$ and $\mu_{v4}=\mu_{34}\,.$

In either case, the marginal distribution $P(x_\SS)$ can be represented as:

\begin{align} \label{eq:k3}
P(x_1,x_2,x_3,x_4) & = \frac{1}{2^4} \left[ 1+ \sum_{\substack{\{i,j\}\subseteq\{1,\cdots,4\}\\ i\neq j}} x_i x_j \mu_{ij}+ x_1 x_2 x_3 x_4\prod_{m\in G^*(\{1,2,3,4\})}\mu_m\right]\,.
\end{align}
$G^*(\{1,2,3,4\})$ entirely contains the dependence of $P(x_1,x_2,x_3,x_4)$ on the underlying tree structure. Finding $G^*(\{1,2,3,4\})$ is equivalent to determining which quartet among $(12|34)\,,(13|24)$ or $(14|23)\,$ corresponds to the underlying structure. As an example if $\T_{|\SS}=\T_5,$ then $G^*(\{1,2,3,4\})$ chooses quartet $(12|34)$ whereas if $\T_{|\SS}=\T_4,$ then $G^*(\{1,2,3,4\})$ is either of $(12|34)\,,(13|24)$ or $(14|23)\,.$ 

Regardless of the matching defined by $G^*(\{1,2,3,4\})$, $\prod_{m\in G^*(\{1,2,3,4\})}\mu_m$ is robust to small variations in  pairwise end-to-end correlations. Lemma \ref{l:robustMatching} clarifies this statement rigorously.


%If the pairwise correlations are noisy,  $G^*(\{1,2,3,4\})$ might choose the incorrect matching, but this only happens when $\prod_{m\in G^*(\{1,2,3,4\})}\wtmu_m$ is close to $\prod_{m\in G^*(\{1,2,3,4\})}\mu_m\,.$ 
\end{ex}



==> App-proof.tex <==
\section{Proofs}

\subsection{Optimal matchings and cherries}
The next two lemmas concern optimal matchings and cherries. For the definition of cherry refer to Subsection~\ref{ss:subtrees}.


If $M\in M_{\CC}$, then for $u\in \CC$ let $M(u)$ denote the match of $u$ in $M$. This means that $\{u,M(u)\}\in M$ for any $u\in \CC$.  
For a matching $M\in M_{\CC}$ (such that $u\in\CC$), define $\Mcadd{ M}{u}{i}=\{ M,\{i,M(u)\}\}\setminus\{u,M(u)\}\,$ to be the matching obtained from $M$ by removing pair $\{u,M(u)\}$ and adding pair $\{i,M(u)\}$.

\begin{lem}\label{l:matching-addnode}
Let $i,j$ be the leaves in a cherry in a tree $\T=(\VV,\EE)$ with parent node $u$. 
For any set of nodes $\CC\in\VV\setminus \{i,j,u\}$ with odd cardinality, replacing $u$ by $i$ results in an optimal matching: $M =G^*(\CC\cup\{u\})$ then $\Mcadd{M}{u}{i}\in G(\CC\cup\{i\})$. 
\end{lem}

\begin{proof}

Note that the sets of matchings $\Mc_{\CC\cup\{i\}}$ and $\Mc_{\CC\cup\{u\}}$ are in bijection via the map $M\mapsto \Mcadd{ M}{i}{u}$ with inverse $M\mapsto \Mcadd{ M}{u}{i}$

%Note that there is a simple one-to-one map between all the matchings $ M'\in M_{\CC\cup\{u\}}$ and $ M''\in M_{\CC\cup\{i\}}$ by choosing $ M''=\Mcadd{ M'}{u}{i}$ and $ M'=\Mcadd{ M''}{i}{u}\,.$

Since $\{i,j,u\}$ form a cherry with $u$ as the parent, for all $v\in\VV\setminus\{i,j,u\}\,,$ $u\in\path_{\T}(i,v)$ and $u\in\path_{\T}(j,v)\,.$ Thus, $\mu_{iv}=\mu_{iu}\mu_{uv}\,.$ Also for all $ M'\in\Mc_{\CC\cup\{i\}}$ and $$ \prod_{m\in M'}|\mu_m|=|\mu_{iu}|\mkern-5mu\prod_{m\in M'_{i\to u}}|\mu_m|$$


For $ M=G^*(\CC\cup\{u\})\,,$ and all $ M'\in\Mc_{\CC\cup\{i\}}\,,$  such that $ M'\neq M_{u\to i}$ or equivalently $ M'_{i \to u}\neq M$
\begin{align*}
\prod_{m\in M'} |\mu_m| & = |\mu_{iu}|\mkern-5mu\prod_{m\in M'_{i\to u}} \mkern-5mu|\mu_m| 
 \leq |\mu_{iu}|\prod_{m\in M} |\mu_m|
 =\mkern-8mu \prod_{m\in M_{u\to i}} \mkern-5mu|\mu_m|\,.
\end{align*}
The above inequality uses the definition given in ~\eqref{e:defG} and $\prod\limits_{m\in M}|\mu_m|\geq \prod\limits_{m\in M''}|\mu_m|$ for all $M''\in \Mc_{\CC\cup\{u\}}\,.$
\end{proof}

\begin{lem}\label{l:matching-addcherry}
Let $i,j$ be the leaves in a cherry in a tree $\T=(\VV,\EE)$ with parent $u$.
For any $\CC\in\VV\setminus \{i,j,u\}$ with $|\CC|=2t$ we have the following property:
  $G(\CC\cup\{i,j\})=G(\CC)\cup\{i,j\}$ i.e., the pair $\{i,j\}$ is matched in the optimal matching of $\CC\cup\{i,j\}\,.$
\end{lem}
\begin{proof}
Since $i,j$ form a cherry with parent $u$, for all the nodes $v\in\CC\,, \mu_{iv}=\mu_{iu}\mu_{uv}\,.$

For any $ M\in\Mc_{\CC\cup\{i,j\}}$ such that $\{i,j\}\notin M$, let $i',j'\in\CC$ be the nodes such that $\{i,i'\}\in M$ and $\{j,j'\}\in M\,.$ So, $\mu_{ii'}=\mu_{iu}\mu_{ui'}$ and $\mu_{jj'}=\mu_{ju}\mu_{uj'}\,.$ Let $ M'=G^*(\CC)\,.$
Then,
\begin{align*}
\prod_{m\in M}|\mu_m| & = |\mu_{ii'} \mu_{jj'}| \prod_{m\in M\setminus\{\{i,i'\},\{j,j'\}\}}|\mu_m|\\
& = |\mu_{iu}\mu_{ui'} \mu_{ju}\mu_{uj'}| \prod_{m\in M\setminus\{\{i,i'\},\{j,j'\}\}}|\mu_m|\\
& \stackrel{(a)}{\leq} |\mu_{ij}|\, |\mu_{i'j'}| \prod_{m\in M\setminus\{\{i,i'\},\{j,j'\}\}}|\mu_m|\\
%%& \leq |\mu_{ij}|\, |\mu_{i'j'}| \prod_{m\in M\setminus\{\{i,i'\},\{j,j'\}\}}|\mu_m|\\
& \stackrel{(b)}{\leq} |\mu_{ij}| \prod_{m\in M'}|\mu_m| =  \prod_{m\in M'\cup\{i,j\}}|\mu_m|
\end{align*}
where (a) uses $\path_{\T}(i'j')\subseteq \path_{\T}(ui') \cup \path_{\T}(uj')$ to get $|\mu_{ui'} \mu_{uj'}|\leq |\mu_{i'j'}|$ and $u\in\path_{\T}(i,j)$ to get $\mu_{ij}=\mu_{iu}\mu_{ju}\,.$ (b) uses the definition~\eqref{e:defG} for $M'=G^*(\CC)\,.$
\end{proof}

\begin{lem} \label{l:marginal3}
For any tree $\T\,,$ the marginal over nodes $\SS=\{1,2,3\}$ satisfies:
\begin{align*} 
P(x_1,x_2,x_3) & = \frac{1}{2^3} \bigg( 1+ \sum_{\substack{\{i,j\}\subseteq\{1,2,3\}\\ i\neq j}} x_i x_j \mu_{ij}\bigg)
\end{align*}
\end{lem}
\begin{proof}
As stated in Section \ref{s:examples}, the induced subtree $\T_{|\{1,2,3\}}$ would be automorphic to either $\T_1$ or $\T_2$ in Figure \ref{fig:marginalTrees}. When $\T_{|\{1,2,3\}}=\T_1\,,$ we would have $X_1\indep X_3 |X_2\,.$ Using total probability lemma, we would have 
\begin{align*}
P(x_1, x_2, x_3)& = P(x_2) P(x_1| x_2) P(x_3| x_2) \\
&= \frac{1}{2} \frac{1+x_1 x_2\mu_{12}}{2} \frac{1+x_2 x_3\mu_{23}}{2} \\
& = \frac{1}{8}\left[1+x_1 x_2\mu_{12} + x_2 x_3\mu_{23}+x_1 x_3\mu_{12}\mu_{23}\right]
\end{align*}
which gives the desired form as $\mu_{12}\mu_{23}=\mu_{13}\,.$

When $\T_{|\{1,2,3\}}=\T_2\,,$ we would have $X_1, X_2$ and $X_3$ are jointly independent conditional on $X_u\,.$ Hence,
\begin{align*}
P(x_1, x_2, x_3) & = \sum_{x_u\in\{-,+\}}P(x_u)\prod_{i=1}^3 P(x_i| x_u) \\
&= \sum_{x_u\in\{-,+\}}\frac{1}{2} \prod_{i=1}^3\frac{1+x_i x_u\mu_{iu}}{2}
\\
& = \frac{1}{8}\left[1+x_1 x_2\mu_{1u}\mu_{2u} + x_2 x_3\mu_{2u}\mu_{3u}+x_1 x_3\mu_{1u}\mu_{3u}\right]\,.
\end{align*}
which gives the desired form as $\mu_{1u}\mu_{2u}=\mu_{12}\,, \mu_{1u}\mu_{3u}=\mu_{13}$ and $\mu_{2u}\mu_{3u}=\mu_{23}\,.$
\end{proof}

\begin{lem} \label{l:robustMatching}
For any set $\CC\subseteq\VV$ with $|\CC|=2t\,,$ and any pair of tree structured Ising distributions $P$ and $Q$ as in ~\eqref{e:Ising} (with possibly different underlying tree), let $\mu_{ij}=\Ex_P X_i X_j$ and $\wtmu_{ij}=\Ex_Q X_i X_j\,.$
If $|\mu_{ij}-\wtmu_{ij}|\leq \epsilon$ for all $i,j\in\CC\,,$ then $$|\mkern-10mu\prod_{m\in G^*(\CC,P)}\mkern-10mu\mu_{m}-\mkern-10mu\prod_{m'\in G^*(\CC,Q)}\mkern-10mu\wtmu_{m'}|\leq 2t\epsilon\,.$$
\end{lem}

\begin{proof}
First, we will show that for all $M\in\Mc_{\CC}\,,$ $\prod_{m\in M}\mu_m$ takes the same sign (\textit{i.e., for $M,M'\in\Mc_{\CC}\,, \prod_{m\in M}\mu_m \prod_{m'\in M'}\mu_{m'}\geq 0$}). Similar statement holds for $\wtmu\,.$
To do so, note that for all $M,M'\in\Mc_{\CC}\,,$ one can make a sequence of matchings $M_0=M, M_1, \cdots, M_r=M' $ such that $M_r$ and $M_{r+1}$ differ only at two pairs of nodes (\textit{i.e.,} There exists $(i,j), (k,l)\in M_r$ such that $(i,k), (j,l)\in M_{r+1}$).  Looking at tree $\T_6$ in Figure \ref{fig:marginalTrees}, it is clear that for the product of correlations on $M_r$ and $M_{r+1}$ have the same sign (\textit{i.e.,} $\prod_{m\in M_r}\mu_m \prod_{m\in M_{r+1}}\mu_m \geq 0$). The same argument applies for all $r$ and hence $\prod_{m\in M}\mu_m \prod_{m'\in M'}\mu_{m'}\geq 0\,.$

Next, we show that if $|\mu_{ij}-\wtmu_{ij}|\leq \epsilon$ for all $i,j\in\CC$, then for any $M=\{m_1, m_2, \cdots, m_t\}\in\Mc_{\CC}\,, |\prod_{m\in M}\mu_m - \prod_{m'\in M}\wtmu_{m'}|\leq t\epsilon\,.$  
\begin{align*}
|\prod_{i=1}^t\mu_{m_i}-\prod_{i=1}^t\wtmu_{m_i}| &= |\sum_{i=1}^t \prod_{j=1}^{i-1}\mu_{m_j}\prod_{j'=i+1}^{t}\wtmu_{m_{j'}} (\mu_i-\wtmu_i)|\\
&\leq \sum_{i=1}^t |\prod_{j=1}^{i-1}\mu_{m_j}\prod_{j'=i+1}^{t}\wtmu_{m_{j'}} (\mu_i-\wtmu_i)|\\
&\leq \sum_{i=1}^t |\mu_i-\wtmu_i|\leq t\epsilon\,.\\
\end{align*}
Let's define $$a =\mkern-18mu\prod_{m\in G^*(\CC,P)}\mkern-10mu\mu_{m}, 
\quad a'=\mkern-18mu\prod_{m\in G^*(\CC,Q)}\mkern-10mu\mu_{m}, 
\quad b =\mkern-18mu\prod_{m\in G^*(\CC,P)}\mkern-10mu\wtmu_{m}, 
\quad b' = \mkern-18mu\prod_{m\in G^*(\CC,Q)}\mkern-10mu\wtmu_{m}\,.$$  Hence, we showed that $a a'\geq 0\,, b b'\geq 0, |a-b|\leq t\epsilon $ and $ |a'-b'|\leq t\epsilon\,.$ We also know that $|a|\geq |a'|$ and $|b'|\geq |b|$ according to the definition of $G^*(\CC,P)$ and $G^*(\CC,Q)\,.$ To bound $|a-b'|\,,$ we study two different cases: Either $a b \geq 0$ in which case $|a-b'| = ||a|-|b'||=\leq \max\{|a-b|,|a'-b'|\}\leq t\epsilon\,$ Or $a b \leq 0$ in which case $|a-b'|=|a|+|b'|\leq |a-b|+|a'-b'|\leq 2 t \epsilon\,.$
\end{proof}
\subsection{Proof of Theorem \ref{t:decomposition}}
\label{s:proofDecomposition}
We use induction on the size of the marginal to prove Equation~\eqref{e:decomposition}. Let $|\SS|=k\,.$ For $P(x)$ described as in Equation~\eqref{e:Ising}, the singleton marginal over any node is uniform distribution. Hence for  $\SS=\{i\}\in\VV$ and $k=1\,,$ $P(x_\SS)=\frac{1}{2}\,.$ 
Additionally, for $\SS=\{i,j\}$ looking at~\eqref{e:Ising},  $P(x_i,x_j)=\frac{1}{4}[1+x_i x_j \mu_{ij}]\,$ which is  the same form given in~\eqref{e:decomposition} for $k=2\,.$

Now assuming that the Equation~\eqref{e:decomposition} holds for all $\CC\subset\VV$ with $|\CC|\leq k-1\,,$ we show that it holds for any given $\SS\subseteq\VV$ with $|\SS|=k\,.$
 
 Looking at subtree $\T_{|\SS}$, we pick nodes $i,j\in\SS$ such that $i$ and $j$ are the leaves of a cherry with parent $u$ such that $u\notin\SS\,.$
  Note that this assumption  is without loss of generality. If the subtree $\T_{|\SS}$ does not have a cherry with nodes $i,j\in\SS\,,$ we can pick a leaf $i\in\SS$ such that there exists a node $j\in\SS$ and $(i,j)\in\T_{|\SS}$ and hence all  paths from $i$ to the nodes in $\SS$ go through $j\,.$ We can  introduce a virtual node $u\notin\VV$ and construct an equivalent tree in which $i,j\in\SS$ are the leaves of a cherry with parent $u\notin\SS$ by replacing $u$ with $j$ and defining $\mu_{uj}=1$ and $\mu_{ui}=\mu_{ij}\,.$
%  Note that the assumption of $u\notin\SS$ is without loss of generality. If the subtree $\T_{|\SS}$ is such that all its leaves do not form a cherry with a parent $u\notin\SS\,,$ we can use a \textit{virtual node} $u\notin\VV$ such that two nodes $\{i,j\}\in\SS$ form a cherry with parent $u$. Then $u$ is connected to the subtree $\T_{|\SS}$ similar to the way $i$ and $j$ was connected to the subtree.
   We define $\RR=\SS\setminus \{i,j\}\,.$
 
 
 Since $i$ and $j$ form a cherry in subtree $\T_{|\SS}$ with parent $u\notin\SS\,,$ we know that $X_i,X_j$ are statistically independent of $ X_{\RR}$ condition on $X_u\,.$
 
Expanding out the probabilities (law of total probability) gives
\begin{align}
P(x_\SS) & = P(x_{\RR},x_i,x_j)\notag\\
& =  P(x_{\RR},x_u=+)P(x_{i}|x_u=+)P(x_j|x_u=+)\notag\\
& \quad+ 
P(x_{\RR},x_u=-)P(x_{i}|x_u=-)P(x_j|x_u=-)\notag\\
& = P(x_{\RR},x_u=+)\cdot\frac{1+x_{i}\mu_{iu}}{2}\cdot \frac{1+x_{j}\mu_{ju}}{2}\notag+ 
P(x_{\RR},x_u=-)\cdot\frac{1-x_{i}\mu_{iu}}{2}\cdot \frac{1-x_{j}\mu_{ju}}{2}\notag\\
& = \frac{1}{4}\left(1+x_{i}x_j \mu_{iu} \mu_{ju}\right)\left[P(x_{\RR},x_u=+)+P(x_{\RR},x_u=-)\right] \notag\\
& \,\, +\frac{1}{4} \left(x_{i}\mu_{iu}+x_j \mu_{ju}\right)\left[P(x_{\RR},x_u=+)-P(x_{\RR},x_u=-)\right]\,. \label{e:totalprob}
\end{align}
Using the assumption of induction~\eqref{e:decomposition} for the set $\RR\cup\{u\}$ with cardinality $k-1$ provides $P(x_\RR,x_u=+)$ and $P(x_\RR,x_u=-)\,.$ We decompose the expression in~\eqref{e:decomposition} into two terms; The first terms considers is the summation of all terms which does not have $x_u$ as a factor. The second term is all the terms that contain $x_u$ as a factor:

\begin{align*}
P(x_\RR,x_u=+) & = \frac{1}{2^{k-1}}\left[\sum_{t=0}^{\lfloor \frac{k-2}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr}
+ \sum_{t=1}^{\lfloor \frac{k-1}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t-1}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC\cup\{u\})} \mu_{\pr}   \right]\\
P(x_\RR,x_u=-) & = \frac{1}{2^{k-1}}\left[\sum_{t=0}^{\lfloor \frac{k-2}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr}
- \sum_{t=1}^{\lfloor \frac{k-1}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t-1}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC\cup\{u\})} \mu_{\pr}   \right] \,.
\end{align*}
Plugging into~\eqref{e:totalprob} gives
\begin{align}\label{e:proofplug4}
P(x_{\SS}) & =  \frac{1}{2^{k}}\left(1+x_{i}x_j \mu_{iu} \mu_{ju}\right)\cdot\sum_{t=0}^{\lfloor \frac{k-2}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr}\notag\\ 
& \quad + 
\frac{1}{2^k}\left(x_{i}\mu_{iu}+x_j \mu_{ju}\right) \sum_{t=1}^{\lfloor \frac{k-1}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t-1}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC\cup\{u\})} \mu_{\pr}\,.
\end{align}

For $\CC\in\RR$ and $|\CC|=2t$, using Lemma \ref{l:matching-addcherry}, $\{i,j\}\cup G^*(\CC)\in G(\CC\cup\{i,j\})$. Also, note that $u\in\path_{\T}\{i,j\}$ and $\mu_{iu}\mu_{ju}=\mu_{ij}$. Hence 
\begin{equation}\label{e:proofplug1}
x_i x_j\mu_{iu}\mu_{ju}\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr} = \prod_{c\in\CC\cup\{i,j\}}x_c\prod_{\pr\in G^*(\CC\cup\{i,j\})} \mu_{\pr}\,.
\end{equation}

For $\CC\in\RR$ and $|\CC|=2t-1$, let $ M= G^*(\CC\cup\{u\})$. Lemma \ref{l:matching-addnode} shows that $\Mcadd{ M}{u}{i}\in G(\CC\cup\{i\})\,:$

% $G(\CC\cup,\{i\})= G(\CC\cup\{u\})\cup\{\}\setminus $. Also, note that $\mu_{iu}\mu_{ju}=\mu_{ij}$. Hence
 
  \begin{equation}\label{e:proofplug2}
  x_i\mu_{iu}\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC\cup\{u\})} \mu_{\pr} = \prod_{c\in\CC\cup\{i\}}x_c\prod_{\pr\in G^*(\CC\cup\{i\})} \mu_{\pr}\,.
    \end{equation}

Similarly,
  \begin{equation}\label{e:proofplug3}
  x_j\mu_{ju}\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC\cup\{u\})} \mu_{\pr} = \prod_{c\in\CC\cup\{j\}}x_c\prod_{\pr\in G^*(\CC\cup\{j\})} \mu_{\pr}\,.
  \end{equation}
  
Plugging~\eqref{e:proofplug1}, \eqref{e:proofplug2}, and~\eqref{e:proofplug3} into Equation~\eqref{e:proofplug4}, gives
\begin{align*}
P(x_\SS) & =\frac{1}{2^k} \left[\sum_{t=0}^{\lfloor \frac{k-2}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr} \right.\\
&\quad
+
\sum_{t=0}^{\lfloor \frac{k-2}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t}} \,\,\prod_{c\in\CC\cup\{i,j\}}x_c\prod_{\pr\in G^*(\CC\cup\{i,j\})} \mu_{\pr}\\
&\quad+ \sum_{t=1}^{\lfloor \frac{k-1}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t-1}} \,\,\prod_{c\in\CC\cup\{j\}}x_c\prod_{\pr\in G^*(\CC\cup\{j\})} \mu_{\pr}\\
&\quad+
\left.\sum_{t=1}^{\lfloor \frac{k-1}{2}\rfloor} \,\sum_{\substack{\CC\subset\RR\\ |\CC|=2t-1}} \,\,\prod_{c\in\CC\cup\{i\}}x_c\prod_{\pr\in G^*(\CC\cup\{i\})} \mu_{\pr}\right]\\
& \stackrel{(a)}{=} \frac{1}{2^k}\left[\sum_{t=0}^{\lfloor k/2\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC)} \mu_{\pr}\right]\,.
\end{align*}
where (a) takes the summation over four different terms: the first term does not have either $x_i$ nor $x_j\,.$ The second terms has both $x_i$ and $x_j\,.$ The third term has $x_j$ but not $x_i\,.$ The fourth terms has $x_i$ but not $x_j\,.$
\subsection{Proof of Proposition \ref{prop:ssTVwithcorr}}

For $i,j\in\VV\,,$ let $\mu_{ij}\triangleq \Ex_{P}X_iX_j$ and $\wtmu_{ij}\triangleq \Ex_{P}X_iX_j\,.$ We also use the notation $G^*(\CC,P)$ to be optimal matching $G^*(\CC)$ under the distribution $P\,.$

To bound $\SS\subseteq\VV$ with $|\SS|=k\,,$ we use Lemma \ref{l:robustMatching} to get: \begin{align*}
d_\mathrm{TV} (P_\SS,Q_\SS) & = \sum_{x_\SS\in\{-,+\}^k} |P(x_\SS)-Q(x_\SS)|\notag\\
& = \frac{1}{2^k}\mkern-5mu\sum_{x_\SS\in\{-,+\}^k} \bigg| \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC,P)} \mu_{\pr} - \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}} \,\,\prod_{c\in\CC}x_c\prod_{\pr\in G^*(\CC,Q)} \wtmu_{\pr} \bigg|\notag\\
& \leq  \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}}\frac{1}{2^k}\mkern-5mu\sum_{x_\SS\in\{-,+\}^k} \,\,\bigg| \prod_{c\in\CC}x_c \bigg| \,\cdot\,\bigg|\prod_{\pr\in G^*(\CC,P)} \mu_{\pr} - \prod_{\pr\in G^*(\CC,Q)}\wtmu_{\pr} \bigg|\\
& =  \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}} \,\,\bigg|\prod_{\pr\in G^*(\CC,P)} \mu_{\pr} - \prod_{\pr\in G^*(\CC,Q)}\wtmu_{\pr} \bigg|\\
&\leq \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} \,\sum_{\substack{\CC\subset\SS\\ |\CC|=2t}} 2t\eta \leq \sum_{t=0}^{\lfloor \frac{k}{2}\rfloor} {k \choose 2t} 2t\eta \leq k2^k \eta\,.\qed
\end{align*}
%Using the telescoping sum for $|a_i|\leq 1$ and $|b_i|\leq 1$ and $|a_i-b_i|\leq \eta$ to get $$|\prod_{i=1}^{t}a_i-\prod_{i=1}^{t}b_i|=|\sum_{i=0}^{t}\prod_{j=1}^{i-1}a_j\prod_{j=i+1}^{t}b_j\,(a_i-b_{i})|\leq t\eta$$ 
%gives for $\CC$ with $|\CC|=2t\,,$ and any matching $M\in\Mc_{\CC}\,,$ 
%$\bigg|\prod_{\pr\in M} \mu_{\pr} - \prod_{\pr\in M}\wtmu_{\pr} \bigg| \leq 2t\eta\,.$
%
%For the sequences $a_i$ and $b_i$ such that $|a_i-b_i|\leq \epsilon\,,$ for all $i\,,$ $\max_i a_i\geq a_j \geq b_j-\epsilon$ which gives $\max_i a_i\geq \max_{i}b_i -\epsilon$ and similarly $\max_i b_i\geq \max_{i}a_i -\epsilon\,.$ Hence, 
%
%$$ \bigg|\prod_{\pr\in G^*(\CC,P)} \mu_{\pr} - \prod_{\pr\in G^*(\CC,Q)}\wtmu_{\pr} \bigg|= \bigg|\max_{M\in\Mc_{\CC}}\prod_{\pr\in M} \mu_{\pr} - \max_{M\in\Mc_{\CC}}\prod_{\pr\in M}\wtmu_{\pr} \bigg|\leq 2t\eta\,.$$



==> GraphTheoryProof.tex <==

\begin{lemma}\label{l:edgePair}
	Let $\T$ and $\Th$ be two spanning trees  such that for a pair of nodes $w,\wt$ we have $\path_{\T}(w,\wt)\neq \path_{\Th}(w,\wt)$. Then, theres exists pairs of edges $f\triangleq (u,\ut)\in \path_{\T}{(w,\wt)}$ and $g\triangleq (v,\vt)\in \path_{\Th}{(w,\wt)}$ such that 
	\begin{enumerate}
		\item[(i)] 	$f\notin \path_{\Th}{(w,\wt)}$ and $g\notin \path_{T}{(w,\wt)}$
		\item[(ii)]  $f\in \path_{\T}{(v,\vt)}$ and $g\in \path_{\Th}{(u,\ut)}$
		%		\item[(iii)] $g \in \path_{\Th}{(u,\ut)}$
	\end{enumerate}
\end{lemma}
 
Since $f\in\path_{\T}(w,\wt)$ and $f\in \path_{\T}{(v,\vt)}$, we can choose the labeling of the end points of the edges $f=(u,\ut)$ and $g=(v,\vt)$ such that $u,v\in \subT{\T}{f}{w}$ and $\ut,\vt\in \subT{\T}{f}{\wt}$. %Additionally, since $f\in \path_{\T}{(v,\vt)}$, the nodes $v$ and $\vt$ are in two different subtrees of the tree $T$ after removing the edge $f$. Thus, we can choose the labeling of the end points of the edge $g=(v,\vt)$ such that $v\in \subT{\T}{f}{w}$ and $\vt\in \subT{\T}{f}{\wt}$.

	\begin{figure}
			\begin{center}
				\includegraphics[width=3in]{fig_proof2.pdf}
				\caption{}
				\label{f:proof2}
			\end{center}
		\end{figure}
\begin{proof}
The proof of this lemma is rather long and does not capture much insight into the main contributions of this paper. The proof is published in a longer version of the paper.
	Let's define a graph $G$. The nodes on this graph are the nodes in $\path_{\T}(w,\wt)\cup \path_{\Th}(w,\wt)$. We define two types of edges in this graph corresponding to the edges in $\path_{\T}(w,\wt)$  and the edges in $\path_{\T}(w,\wt)$. Then, we merge any pair of nodes between which there are two types of edges. Note that since $\path_{\T}(w,\wt)\neq \path_{\Th}(w,\wt)$, the nodes $w$ and $\wt$ will not be merged with each other during this process. We call the remaining nodes  and edges in $\path_{\T}(w,\wt)$, $u_1,u_2,\cdots,u_{K-1}$ and $f_1,f_2,\cdots,f_K$ correspondingly.  Similarly, we call the remaining nodes  and edges in $\path_{\Th}(w,\wt)$, $v_1,v_2,\cdots,v_{L-1}$ and $g_1,g_2,\cdots,g_L$ correspondingly. Where that $K$ and $L$ are positive integers. We define these edges so that the two nodes connected by $f_k$ and $g_l$ are $f_k=(u_{k-1},u_k)$ and $g_l=(v_{l-1},v_l)$. This notation is consistent if we define $u_0 = v_0 = w$ and $u_K = v_L = \wt$. Note that in this notation one nodes can have several labels depending on the context. 
	
	According to the definition, we know that  $f_k\in \path_{\T}(w,\wt)$ and $g_l\in \path_{\Th}(w,\wt)$ for all $k=1,\cdots,K$ and $l=1,\cdots,L$. The process of merging nodes as described guarantees that $f_k\notin \path_{\Th}(w,\wt)$ and $g_l\notin \path_{\T}(w,\wt)$. Thus, in order to prove the existence of edges with the properties given in the lemma, all we have to do is to find  a pair of edges $f_{k^*}$ and $g_{l^*}$ such that $f_{k^*}\in \path_{\T}{(v_{l^*-1},v_{l^*})}$ and $g_{l^*}\in \path_{\Th}{(u_{k^*-1},u_{k^*})}$.  
	
	Now we define another graph $\widehat{G}$ to be the graph with the nodes $\widehat{\VV}=\{w,\wt,u_1,u_2,\cdots,u_K,v_1,v_2,\cdots,v_L\}$. There are two types of edges in this graph corresponding to the connectivity in the spanning tree $\T$ and $\Th$. We denote the edges corresponding to the tree $\T$ by $\EE$ and the edges corresponding to the tree $\Th$ by $\widehat{\EE}$. 
	Consequently, $\EE$ and $\widehat{\EE}$ both construct two different spanning trees of the graph $\widehat{G}$ on the nodes $\VV$. 

	The set of edges $\EE$ determine a spanning tree denoted by $\St$ and satisfy all the conditional independence properties satisfied by the original spanning tree $\T$ on the nodes $\widehat{\VV}$. Concretely, any pair of nodes $(i,j)$ in $\widehat{\VV}$ are connected by an edge in $\EE$ if and only if all the nodes in $\path_{\T}(i,j)$ have been removed from $\VV$ during construction of $\widehat{G}$, i.e., $\widehat{\VV} \cap \path_{\T}(i,j) = \{i,j\}$.
	
	 Similarly, the edges $\widehat{\EE}$ are chosen so that the spanning tree implied them, denoted by $\Sth$ satisfies all the conditional independence properties satisfied by the original spanning tree $\Th$. 
	
	%For $k=1,\cdots,k$, we define the two nodes connected by edge $f_k$ to be $f_{k}=(u_{k-1},u_{k})$. This notation is consistent with the previous definition of $u_{k}$'s if we define $u_{0}=w$ and $u_{K}=\wt$. 
%	\GB{Easiest to just do this preceding bit in the first place and remove redundancy.}
	We define the set $\D_{k}=\{l;\; g_l \in \path_{\Sth}(w,\wt)\cap \path_{\Sth}(u_{k-1},u_k)\}$ to be the set of edges in $\path_{\Sth}(w,\wt)$ which are also in the path connecting the two ends of $f_k$ in the tree $\Sth$. Similarly, for $l=1,\cdots,L$ we define the sets $\C_l=\{k;\; f_k \in \path_{\St}(w,\wt)\cap\path_{\St}(v_{l-1},v_l)\}$. 
	\MK{Two figures are suggested for this proof.}
	If there exists the pair integers $k^*$ and $l^*$ such that $l^*\in\D_{k^*}$ and $k^*\in\C_{l^*}$, then they correspond to the edges $f_{k^*}\in \path_{\T}{(v_{l^*-1},v_{l^*})}$ and $g_{l^*}\in \path_{\Th}{(u_{k^*-1},u_{k^*})}$.  As stated previously, this pair of edges satisfy all the properties given in the lemma.
	
	To find such pair of $l$ and $k$ we prove a ``no gap" property of the sets $\{\C_{l}\}$, with a similar statement holding for $\{\D_{k}\}$. We will use the following notation in the statement of the ``no gap" lemma. Let's define 
	\begin{eqnarray*}
	\underline{\D}_{k'} &= \bigcup_{k=1}^{k'} \D_k, \quad \overline{\D}_{k'} &= \bigcup_{k=K-k'}^{K} \D_k\\
\underline{\C}_{l'} &= \bigcup_{l=1}^{l'} \C_l, \quad \overline{\C}_{l'} &= \bigcup_{l=L-l'}^{L} \C_l.
		\end{eqnarray*}
	
	\begin{lemma}[``No gap" lemma]\label{l:noGap}
		For any $l'>0$, if $\underline{\C}_{l'}\neq \varnothing$, there exists $k'>0$ such that $\underline{\C}_{l'}=\{1,2,\cdots,k'\}$. 	For any $l'>0$, if $\overline{\C}_{l'}\neq \varnothing$, then there exists $k'\geq 0$ such that $\overline{\C}_{l'}=\{K-k',\cdots,K\}$. 
	\end{lemma}
	
	To prove that the ``no gap" property of the sets $\{\C_{l}\}$ and $\{\D_{k}\}$, we define the following function $\textsf{M}: \{0,1,2,\cdots,K\}\to \{-1,0,1,2,\cdots,K\}$ such that $\textsf{M}(0)=-1$ and for $1\leq k'\leq K$, 
	\begin{equation}\label{eq:funcM}
	{M}(k')=\max\{i; i\in \cup_{l\in \underline{\D}_{k'}}\C_l\}.
		\end{equation}
			% $\underline{\D}_{k'} = \cup_{k=1}^{k'} \D_k$.
Note that $\underline{\D}_{k'} \subseteq \underline{\D}_{k'+1} $ and consequently $\cup_{l\in \underline{\D}_{k'}}\C_l \subseteq \cup_{l\in \underline{\D}_{k'+1}}\C_l$. Thus, 
the function $\textsf{M}(k')$ is non-decreasing over its domain. 
	
	Also, due to the no gap property of the sequence of sets $\{\C_{l}\}$ and $\{\D_{k}\}$, we know that $\underline{\D}_{K}=\{1,\cdots,L\}$ and $\cup_{l=1}^{L}\C_l= \underline{\C}_{L}=\{1,\cdots, K\}$. Thus,  $\textsf{M}(K)=K$.
	Define $$k^*=\min\{k: \, 1\leq k\leq K \,\text{and}  \, k\leq M(k) \}.$$ Thus, we know that $k^* \leq \textsf{M}(k^*)$ and $M(k^*-1)< k^*-1 <k^*$. So, $\textsf{M}(k^*-1)<k^*\leq \textsf{M}(k^*)$. According to the definition given by equation~\eqref{eq:funcM}, there exists some $l^*\in\D_{k^*}$ such that $k^*\in\C_{l^*}$.  
	
	As mentioned before, this pair integers determine the edges that satisfy the properties given in the lemma. 
	%	\GB{Here explain how lemma gives ``, and this implies the existence of a pair of edges $f$ and $g$ with the properties given in the lemma."}
	\end{proof}
\begin{proof}[Proof of Lemma~\ref{l:noGap}]	For each node $v_{l}$ we define a pointer $\pv{l}=\max\{k;\; u_k \in \path_{\St}(w,v_l)\}$. Note that $\pv{0}=0$ and $\pv{L}=K$. Similarly we define the sequence of pointers $\pu{k}=\max\{\{l;\; v_l \in \path_{\Sth}(w,u_k)\}\}.$
	
	These pointers determine the sequence of sets $\C_l$'s (and similarly for $\D_k$'s) as follows: For any $l>0$, if $\pv{l}>\pv{l-1}$, $\C_l= \{\pv{l-1}+1,\cdots,\pv{l}\}$. If $\pv{l}=\pv{l-1}$, then $\C_l=\varnothing$. And if $\pv{l}<\pv{l-1}$, then $\C_l= \{\pv{l}+1,\cdots,\pv{l-1}\}$.
	
	Based on this characterization of the sets $\C_l$'s, the nested version of the sets $\C_l$'s is $$\underline{\C}_{l'}=\Big\{1,\cdots,\max_{l\leq l'}\pv{l}\Big\}\,.$$
	This is nonempty if and only if $\max_{l\leq l'}\pv{l}>0$. Similarly, we have that 
	$$\overline{\C}_{l'}=\Big\{\min_{l\geq L-l'}\pv{l},\cdots,K\Big\}\,.$$
	
	Similar reasoning gives
	$$\underline{\D}_{k'}=\Big\{1,\cdots,\max_{k\leq k'}\pu{k}\Big\}$$
	and
	$$\overline{\D}_{k'}=\Big\{\min_{k\geq K-k'}\pu{k},\cdots,L\Big\}\,.$$
	
	Observe that $\max_{l\leq l'}\pv{l}$ as a function of $0\leq l'\leq L$, is monotonically increasing,  where $\pv{0}=0$ and $\pv{L}=K$. Similarly, $\max_{k\leq k'}\pu{k}$ as a function of $0\leq k'\leq K$, is monotonically increasing, where $\pu{0}=0$ and $\pu{K}=L$. Consequently, there exists a pair of integers $l$ and $k$ such that $k\in\C_{l}$ and $l\in \D_k$.
\end{proof}



==> Pcorr.tex <==

Let $$\EEstrong_{\T}=\{(i,j)\in\EE_{\T};|\tanh(\theta_{i,j})|\geq \frac{4\epsilon}{\sqrt{1-\tanh(\beta)}} \}$$
consist of the set of strong edges in tree $\T$ according to the distrution $P(x)$.

We define the event 
\begin{equation}
\label{e:Pcorr}
\Pcorr = \{(i,j)\in \EE_{\Tc} ; \,\text{for all } \, (i,j)\in \EEstrong_{\T} \}
\end{equation}
where $\Tc$ is the Chow-Liu tree.



\begin{lemma}
\label{l:Pcorr}
With $\eps$ defined in Equation~\eqref{e:Epsilon}, event $\Pcorr$ happens with probability at least $1-\delta$.
\end{lemma}


==> forestProof__Mina_Karzand_s_conflicted_copy_2018-01-27_.tex <==
\subsection{Sample complexity of forest approximation algotithm}

\begin{proof}[Proof of Proposition~\ref{pro:forestLB}]
Since the loss function $\widetilde{d}(P,Q)$ defined in~\eqref{eq:forest-loss} is not symmetric, one cannot use Corollary~\ref{cor:Fano-loss} to find a lower bound for the sample complexity of the forest approximation algorithm.

Define $M=p-1$ models as follows: Let $\theta^1$ be the model in which $\theta^1_{12}=0$ and $\theta^1_{1i}=\beta$ for any $3\leq i \leq p$. For each $m\leq p-1$, define $\theta_m$ such that $\theta^0_{12}=0$, $\theta^0_{1i}=\beta$ for any $3\leq i \leq p$ and $\theta^m_{2,m+1}=\mathrm{atanh}(\eta)$. 
 
 Let $\Phi:\{-1,+1\}^{p\times n}\to 2^{\VV\setminus\{1\}}$ be an estimator that uses $n$ samples to recover the neighborhood of node 1. Let $\Psi'_{\Phi}$ be an estimator that takes $n$ samples and generates a forest $\mathsf{F}$ (which is constrained to have the same neighborhood for node $1$ that the estimator $\Phi$ recovers) and a distribution $Q\in\PP_{\mathsf F}(0,\beta)$. Then
 \begin{align*}
\inf_{\Psi} \sup_{\T\in \TT\atop P\in\PP_{\T}(\al,\beta)} &\P\left[\widetilde{d}\big(P,\Psi(X^{\small(1:n\small)})\big) > \eta\right]  
%= \inf_{\Phi}\inf_{\Psi'_{\Phi}} \sup_{\T\in \TT\atop P\in\PP_{\T}(\al,\beta)} \P\left[\widetilde{d}\big(P,\Psi(X^{\small(1:n\small)})\big) > \eta\right] \\
 \geq
  \inf_{\Phi}\inf_{\Psi'_{\Phi}} \max_{m}\P_{\theta^m}\left[\widetilde{d}\big(P,\Psi(X^{\small(1:n\small)})\big) > \eta\right]\\
  & \geq    \inf_{\Phi} \max_{m}
\,  \inf_{\Psi'_{\Phi}}\,\,
\P_{\theta^m}\left[\widetilde{d}\big(P,\Psi(X^{\small(1:n\small)})\big) > \eta\right]\\
 & \geq    \inf_{\Phi} \max_{m}\,\,
 \P_{\theta^m}\left[\Phi(X^{\small(1:n\small)})\big) \neq \partial_{\theta^m}(1) \right]
 \end{align*}
\end{proof}




Fix $\eta>0$. Let $\Psi$  be an estimator that takes $n$ samples generated from $\P_{\T}(0,\beta)$ and recovers a forest $\mathsf F$ and a distribution $Q\in\P_{\mathsf F}(0,\beta)$. Let the (not-symmetric) distance $\widetilde{d}$ between distributions $P$ and $Q$ be \begin{equation}\label{eq:forest-loss}
\widetilde{d}(P,Q)= \max\big\{\LL^{(2)}(P,Q), {1\!\!1}[\EE_{\mathsf F} \nsubseteq\EE_{\T}]\big\}\,.
\end{equation}
Then if $n<$, then  the worst-case probability of $\widetilde{d}$ loss greater than $\eta$ taken over trees $\T\in \TT$ and distributions $P\in \PP_{\T}(\al,\beta)$ is at least half for any algorithm, i.e., $$\inf_{\Psi}\sup_{\T\in \TT\atop P\in\PP_{\T}(\al,\beta)} \P\left[\widetilde{d}\big(P,\Psi(X^{\small(1:n\small)})\big) > \eta\right]>1/2\,.$$ 

==> hoeffding.tex <==
\section{Hoeffding deviation bound} 
The following lemma is based on Theorem 3 of Hoeffding \cite{hoeffding1963probability}. 
\begin{lemma} \label{l:hoeffd2}
Let $Z^{(1)}, \cdots, Z^{(n)}$ be i.i.d. random variables such that $\Ex{\big[Z^{(i)}\big]}=0,$ $|Z^{(i)}|\leq b$ and $\Ex{\big[(Z^{(i)})^2\big]}\leq \sigma^2$. Let $\bar{Z}=\frac{1}{n}\sum_{i=1}^n Z^{(i)}$. Then
\begin{align}
\Ex{\big[\exp(\lambda \bar{Z})\big]} &\leq \exp\left\{n\,f\Big(\frac{\sigma^2}{b^2} ,\frac{b|\lambda}{n}\Big)\right\},
\end{align}
where we defined 
\begin{equation}
f(u,c)=\log\left(\frac{1}{1+u}e^{-cu}+ \frac{u}{1+u}e^c\right).
\end{equation}
Also, if $c\geq 0$, the function $f(u,c)$ is concave and nondecreasing in $u$ for $u\geq 0$. And for any $t\geq 0,$
\begin{equation} \label{eq:hoeff2-deviation}
\P\Big[|\bar{Z}|> t\Big] \leq 2 \left\{\Big(1+\frac{bt}{\sigma^2}\Big)^{-(1+bt/\sigma^2) \frac{\sigma^2}{b^2+\sigma^2}} \,\Big(1-\frac{t}{b}\Big)^{-(1-t/b) \frac{b^2}{b^2+\sigma^2}} \right\}^n\,.
\end{equation}
\end{lemma}



==> lowerbdSSTV.tex <==
\section{Lower bound for ssTV loss in the extreme case of $\alpha=\beta$}

Here, we provide a lower bound for the ssTV loss in the case $\tanh(\beta)\leq \tanh(\alpha)+2\eta$. In this case, since there is little uncertainty about edge parameters of the model apriori, the incurred loss is due to the incorrect structure recovery rather than the parameter estimation error.

\begin{lemma}

$\tanh(\beta)\leq \tanh(\alpha)+2\eta$ 

\end{lemma}
